Understanding Android Obfuscation Techniques: A Large-Scale Investigation in the Wild

In this paper, we seek to better understand Android obfuscation and depict a holistic view of the usage of obfuscation through a large-scale investigation in the wild. In particular, we focus on four popular obfuscation approaches: identifier renaming, string encryption, Java reflection, and packing. To obtain the meaningful statistical results, we designed efficient and lightweight detection models for each obfuscation technique and applied them to our massive APK datasets (collected from Google Play, multiple third-party markets, and malware databases). We have learned several interesting facts from the result. For example, malware authors use string encryption more frequently, and more apps on third-party markets than Google Play are packed. We are also interested in the explanation of each finding. Therefore we carry out in-depth code analysis on some Android apps after sampling. We believe our study will help developers select the most suitable obfuscation approach, and in the meantime help researchers improve code analysis systems in the right direction.

==> casestudy.tex <==
\section{Case Studies}
\label{sec:case}
In this section, we conduct two case studies to better understand the Android code obfuscation in the wild from the aspects of paralog and timeline.
\subsection{Paralog-based Study}
%\ljian{I like the cross-checking case in this section. More such cases and security implication analysis would make our stronger.}

%\ljian{We could share the findings in a website, so community can validate them and help to further research}

We notice some mobile software companies release a series of apps which contain the same code block or libraries.  Such phenomenon is reasonable for sharing the intellectual resources and reducing the development cost. However, in large enterprises, different apps are usually developed by different teams with differential development standards. To code protection, differential standards may cause obfuscation failure at the company-scale comparison.

For example, Baidu~\cite{url_baidu} is a dominate search engine company in China. It also developed more than 100 Android apps for nearly every aspect, such as Baidu Map, Baidu IME, Baidu Game Box, etc. In the analysis, we find these apps are often applied different obfuscation strategies (or even using different tools).  One direct problem is that a shared class (library) is obfuscated in one app but not in another app. Therefore the obfuscated part could be restored through cross-checking. As shown in Figure~\ref{fig:case_same_developper}, the \texttt{cloudsdk} library is obfuscated in Baidu Dictionary (\texttt{com.baidu.dict}), but not in Baidu Video Player (\texttt{com.baidu.video}). Such "obfuscated" classes will become transparent to attackers.

\begin{figure}[t]
	\centering
	\includegraphics[width=1\columnwidth]{pic/case_same_developper.pdf}           
	\caption{Cross-check -- obfuscated \texttt{cloudsdk} library}
	\label{fig:case_same_developper}
\end{figure}


\subsection{Timeline-based Study}
%\ljian{We need some cases to show other obfuscations than identifier-renaming.}
Similar to the evolution of app functions , the security scheme of an app is also changing. In our analysis, we found that there are some off-the-shelf apps whose previous versions did not pay enough attention to code protection, especially code obfuscation. 

For example, Instagram \cite{url_instagram} is a famous social software. Statistics show that till April 2017, the number of Instagram's active users has reached more than 600 millions \cite{url_statis}. We downloaded 126 different versions of Instagram from v1.0.1 to v10.9.0 and explore the evolution of its obfuscation techniques.

\begin{figure}[t]
	\centering
	\includegraphics[width=1\columnwidth]{pic/timeline.pdf}           
	\caption{Timeline of obfuscation: the case of Instagram}
	\label{fig:timeline}
\end{figure}

From the result we can see that Instagram started using code obfuscation from version 5.0.1. Among all the obfuscation techniques, only identifier-renaming was used. As our previous sections says, identifier-renaming can only provide basic code protection. In our case, we find that non-obfuscated code in older versions can make code in current version vulnerable. We give two code snippets extracted from version 4.0.1 and version 5.0.1 in Appendix~\ref{appendix: time-line}



==> obftech.tex <==
\section{Android Obfuscation Techniques Characterization}
\label{sec:obftech}
In this section, we review several frequently used Android obfuscation techniques and highlight their features.

\vspace{2pt} \noindent 
\textbf{Identifier Renaming.}
In an ordinary non-obfuscated app, identifiers' names are usually meaningful. They may vary in their representations, like \emph{CamelCase}, \emph{Hungarian Notation}, while still comprehensible. Meaningful names are helpful for software development due to their good readability. However, they also accommodate reverse-engineers to rapidly comprehend the purpose of the code and locate target functions. To reduce the potential information leakage, an identifier's name is usually replaced by another meaningless string in an obfuscated app. The following code snippet gives an example. All the identifiers in class \emph{Account} are renamed, increasing the confusion of analysis.


{\small
	\begin{lstlisting}[
	language={Java},
    label={lst:identifier},
	keywordstyle=\color{blue!70},
	xleftmargin=5pt,
	xrightmargin=5pt,
	numberstyle=\scriptsize,
	breaklines=true,
	frame=single,
	%frame=shadowbox,
	basicstyle=\ttfamily,
	commentstyle=\color{blue} \textit,
	stringstyle=\itfamily,
	showstringspaces=false]
public class Account{
    private Integer Age;
    public void setAge(Integer age){
    	this.Age = age;
    }
}
-----------------After Renaming-----------------
public class a{
    private Integer a;
    public void a(Integer a){
    	this.a = a;
    }
}
	\end{lstlisting} 
}



\vspace{2pt} \noindent 
\textbf{String Encryption.}
Strings are very common-used data structures in software development. To prevent the sensitive information from being revealed, strings are usually encrypted in an obfuscated app. Using encryption and decryption functions, original plain texts are mapped to meaningless character combinations and restore at runtime. String encryption can effectively hinder \emph{hard-coded} static scan and enhance the effect of the obfuscation. The following code block shows an example of string encryption.

{\small
	\begin{lstlisting}[
	language={Java},
    label={lst:encryption},
	keywordstyle=\color{blue!70},
	xleftmargin=5pt,
	xrightmargin=5pt,
	numberstyle=\scriptsize,
	breaklines=true,
	frame=single,
	%frame=shadowbox,
	basicstyle=\ttfamily,
	commentstyle=\color{blue} \textit,
	stringstyle=\ttfamily,
	showstringspaces=false]
String option = "@^@#\x `1 m*7 %**9_!v";
this.execute($\textbf{decrypt}$(option));


	\end{lstlisting} 
}


\vspace{2pt} \noindent 
\textbf{Excessive Overloading.} The overloading feature allows different functions share the same name while keeping parameters and implementations varied. It provides more convenience and readability for programming. The following code block gives a simple example of overloading functions.


\dwr{change to a short case}
{\small
	\begin{lstlisting}[
	language={Java},
    label={lst:overloading},
	keywordstyle=\color{blue!70},
	xleftmargin=5pt,
	xrightmargin=5pt,
	numberstyle=\scriptsize,
	breaklines=true,
	frame=single,
	%frame=shadowbox,
	basicstyle=\ttfamily,
	commentstyle=\color{blue} \textit,
	stringstyle=\ttfamily,
	showstringspaces=false]
void printInfo(float b){
	System.out.println(b); 
}
void printInfo(float[] b){
	for(int i=0; i<b.length; i++){
    	System.out.println(b[i]); 
        }
}
	\end{lstlisting} 
}


From the perspective of obfuscation, fields and methods can be changed to one name no matter how irrelevant they are, enhancing the bewilderment and confusion of reverse-engineering. 


\vspace{2pt} \noindent 
\textbf{Java Reflection.} Reflection is an advanced feature provided by Java, which allows programs to modify the runtime behavior running in the Java virtual machine~\cite{url_reflection}. This feature can help developers manipulate Java code dynamically, e.g., creating new object instances and invoking methods dynamically. One legitimate usage is to invoke nonpublic APIs in the SDK (with the label \texttt{@hide}). The following code block gives an example of reflection that invokes a hidden API \texttt{android.os.ServiceManager.getService} function to get \texttt{batteryinfo}.
{\small
	\begin{lstlisting}[
	language={Java},
    label={lst:reflection},
	keywordstyle=\color{blue!70},
	xleftmargin=5pt,
	xrightmargin=5pt,
	numberstyle=\scriptsize,
	breaklines=true,
	frame=single,
	%frame=shadowbox,
	basicstyle=\ttfamily,
	commentstyle=\color{blue} \textit,
	stringstyle=\ttfamily,
	showstringspaces=false]
Object object = new Object();
Method getService = Class.forName("android.os.ServiceManager").getMethod("getService", String.class);
Object obj = getService.invoke(object, new Object[]{new String("batteryinfo")});
	\end{lstlisting} 
}

As an obfuscation technique, reflection is a good choice for hiding app's behaviors since state-of-the-art static analysis tools are still problematic when handling dynamic calls. Therefore, malicious app developers heavily employ reflections to hide malicious actions.

\vspace{2pt} \noindent 
\textbf{Packing.} Packing is a widely-used code protection technique. The packed apk is composed of an encrypted origin apk and a wrapper apk. When the user launch the apk, the wrapper will run first, it will decrypt the origin apk and loads it into the memory, then the execution will be handed to the decrypted apk. Due to the crypto procedure and runtime release, it becomes hard to get the origin code through static analysis. We regard packing as an obfuscation skill in a broad sense for its goal is to hinder the reverse-engineering which is identical to obfuscation.

Many corporations provide free or customized packing services now, like \emph{Bangcle}, \emph{ijiami}, \emph{Qihoo} and \emph{Tencent}, which are very easy to use. What the user needs to do is to upload the APK file, select functionalities they need and wait. The packing procedure usually takes several minutes. After that, the user can download the packed APK, sign it and publish it on the APK market.

